Recommending Deployment Strategies for Collaborative Tasks

Our work contributes to aiding requesters in deploying collaborative tasks in crowdsourcing. We initiate the study of recommending deployment strategies for collaborative tasks to requesters that are consistent with deployment parameters they desire: a lower-bound on the quality of the crowd contribution, an upper-bound on the latency of task completion, and an upper-bound on the cost incurred by paying workers. A deployment strategy is a choice of value for three dimensions: Structure (whether to solicit the workforce sequentially or simultaneously), Organization (to organize it collaboratively or independently), and Style (to rely solely on the crowd or to combine it with machine algorithms). We propose StratRec, an optimization-driven middle layer that recommends deployment strategies and alternative deployment parameters to requesters by accounting for worker availability. Our solutions are grounded in discrete optimization and computational geometry techniques that produce results with theoretical guarantees. We present extensive experiments on Amazon Mechanical Turk and conduct synthetic experiments to validate the qualitative and scalability aspects of StratRec.

==> discussion.tex <==
\section{Discussion}\label{discussion}
We discuss two immediate extension of \StratRec that are part of our ongoing investigation.\\
{\bf Worker availability as pdf:} Instead  of an expected value, one possible  extension is  to use the actual pdf and revisit the problems in \StratRec. This will  require reformulating {\tt Batch Deployment Recommendation} and \ADPaR. For example,  the goal of the former problem would be to optimize  $F$ in an  expected sense, considering $W$ as a pdf.  Similarly, \ADPaR will  produce $k$ different strategies  for every possible worker availability value considering its corresponding probability. We note that the current framework stays unaltered under this extension, only the designed algorithms are likely to exhibit higher computational complexity.

{\bf Non-linear relationship between worker availability and parameters of a strategy:}
\BatchStrat would need to be adapted for the case where the relationship between worker availability and the parameters of a strategy  is non-linear. We note that theoretical guarantees of our designed solutions (\BatchStrat and \ADPaRA) as well as their running time hold on all the polynomial relations with degree less than five, because these functions do have analytical solutions for finding zero points. As for functions with higher degrees, \ADPaRA will remain unaltered. The only change will be for the Workforce Requirement Computation in Section~\ref{wr}, that will rely on the Newton-Raphson method, and hence its running time will increase.


